Breaking Event Rumor Detection via Stance-Separated Multi-Agent Debate

The rapid spread of rumors on social media platforms during breaking events severely hinders the dissemination of the truth. Previous studies reveal that the lack of annotated resources hinders the direct detection of unforeseen breaking events not covered in yesterday's news. Leveraging large language models (LLMs) for rumor detection holds significant promise. However, it is challenging for LLMs to provide comprehensive responses to complex or controversial issues due to limited diversity. In this work, we propose the Stance Separated Multi-Agent Debate (S2MAD) to address this issue. Specifically, we firstly introduce Stance Separation, categorizing comments as either supporting or opposing the original claim. Subsequently, claims are classified as subjective or objective, enabling agents to generate reasonable initial viewpoints with different prompt strategies for each type of claim. Debaters then follow specific instructions through multiple rounds of debate to reach a consensus. If a consensus is not reached, a judge agent evaluates the opinions and delivers a final verdict on the claim's veracity. Extensive experiments conducted on two real-world datasets demonstrate that our proposed model outperforms state-of-the-art methods in terms of performance and effectively improves the performance of LLMs in breaking event rumor detection.

==> reproduce.tex <==
\newpage
\setcounter{secnumdepth}{0}
\section{Reproducibility Checklist}
Unless specified otherwise, please answer ``yes'' to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.

\vspace{0.5cm}
This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
 \textbf{yes}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) \textbf{yes}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) \textbf{yes}
\end{itemize}

\vspace{0.5cm}
\noindent Does this paper make theoretical contributions? (yes/no) \textbf{no}\\
If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\vspace{0.5cm}
\noindent Does this paper rely on one or more datasets? (yes/no) \textbf{yes}\\
If yes, please complete the list below.
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) \textbf{yes}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) \textbf{NA}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) \textbf{NA}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) \textbf{yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) \textbf{yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) \textbf{NA}
\end{itemize}

\vspace{0.5cm}
\noindent Does this paper include computational experiments? (yes/no) \textbf{yes}\\
If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no). \textbf{yes}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) \textbf{yes}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \textbf{yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \textbf{yes}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) \textbf{yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) \textbf{yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) \textbf{yes}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) \textbf{no}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) \textbf{yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) \textbf{no}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) \textbf{yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) \textbf{NA}
\end{itemize}

==> review.tex <==
review1:
Dear Reviewer 4gKb, we sincerely appreciate your invaluable and constructive comments. We respond to your concerns one by one.

Q1: About the prompts used are not very descriptive, could be ambiguous.

The design style of using "Fake" or "Real" as labels for the prompts is common in the rumor detection field, and that this approach aligns with the usual template for applying large models in such tasks. The prompt in A.5, which uses the previous round's responses from other agents, is described in detail in Section 3.4.1 (lines 369-372) of your paper. 

[1] Liu, Q.; Tao, X.; Wu, J.; Wu, S.; and Wang, L. 2024. Can Large Language Models Detect Rumors on Social Media? ArXiv preprint, abs/2402.03916.

[2] Li, X.; Zhang, Y.; and Malthouse, E. C. 2024. Large Language Model Agent for Fake News Detection. ArXiv preprint, abs/2405.01593.


Q2: “Only LLM for each of the datasets in English and Chinese have been explored. It might be useful to replicate some of the results for at least another LLM for each.”

I'm truly sorry, I didn't fully understand this valuable suggestion. I would appreciate any further guidance you can provide.

Q3: " It’s not clear what subjective and objective means from Fig 1 so it’s not really clear at this point in the paper."

In Figure 1, we use the subjective claim "Breaking: A child under the age of 18 has died of coronavirus in Los Angeles, public health officials announce, in a rare and tragic case." as an example. In the figure, the term "Non-subjective" in the middle of the figure is highlighted in bold to indicate that this is a non-subjective claim. Additionally, we provide explanations in sections 3.3.1 "Subjective Expression Claims" and 3.3.2 "Non-subjective Claims."

Q4: “other debaters” is not clear. Isn’t this supposed to be just single-stance comments?

The comments have two positions: supporting the claim and opposing the claim. We first perform Stance Separation (Section 3.2 Stance Separation) on the comments, then use two agents to generate the initial opinion based on different positions using our designed prompt templates. The two agents then engage in a debate to reach a final conclusion. The term "other debaters" in the original text refers to the fact that after the initial opinions are generated by the two agents, each agent debates based on the other’s initial opinion.

Q5: Why speculate that they reach consensus by the 2nd turn? Why not actually check when the consensus takes place and use early stopping?

When exploring the impact of debate rounds on our model's performance, we conducted ablation experiments using 0-5 rounds, as shown in Figure 2. We found that the model performs best in the second round, so we speculate that consensus is reached by the second turn, and we analyze this in Section 4.4.1 "Debate Rounds." Checking when consensus occurs and using early stopping is a great suggestion, as it would save a significant amount of tokens.

Q6: Are only the immediate child nodes of the parent comment used? Or any comments in the tree? If not only the child nodes, the problem is a little more complex when prompting for fake or real post – the comment could be disagreeing with a parent comment that disagrees with the post itself. This could potentially seep in some false positives on either side.

During stance separation, we used all the comments. Our goal was to allow the agents to debate based on different viewpoints. In this process, even if some comments are rebuttals to others, they can provide additional perspectives for the agents, helping the model align more closely with the logical flow of real-world discussions during analysis and judgment.

Q7: Table 2: I wonder why w/o Non-Sub for Weibo performs so well. It might also be useful to include a significance test for if the performance metrics are significantly different from the full model.

Thank you for your valuable feedback. For subjective and non-subjective claims, we employed different prompt strategies to generate the initial opinion. The strong performance of "w/o Non-Sub" for Weibo can be attributed to the higher prevalence of subjective claims in the Weibo-COVID19 dataset. "W/o Non-Sub" indicates that the model uses prompts corresponding only to subjective claims for all claims. Therefore, when subjective claims are more common, "w/o Non-Sub" performs better.


Q8: the error bars for the early detection graphs.

We share your observation in the early detection experiments. Despite the number of trials we conducted, the error remained within 2.3\%, and the overall trend did not change significantly. Additionally, we observed similar outstanding performance in models using other LLMs for social media rumor detection.

[2] Li, X.; Zhang, Y.; and Malthouse, E. C. 2024. Large Language Model Agent for Fake News Detection. ArXiv preprint, abs/2405.01593.


review2:
Dear Reviewer KsrN, we sincerely appreciate your invaluable and constructive comments. We respond to your concerns one by one.

Q1: About the stance of comments on a claim in a social media post.
Thank you for your reviews. Our framework aims to identify comments on a claim that support or oppose it. Comments supporting the claim are assigned to one agent, while those opposing it are assigned to another agent. The two agents then engage in a debate based on the prompt we designed. It does not assume that the stance of comments on a claim in a social media post can determine the veracity of the claim, nor is it based on the amount of support the claim receives.

Q2:About "subjective claims".

Firstly, we recognize that the definition of "subjective claims" in the current paper is somewhat ambiguous, which may lead to unclear concepts. Therefore, we will provide a clearer definition. A "subjective claim" refers to a linguistic expression that reflects an individual perspective, emotion, or value judgment, typically representing personal opinions or feelings. However, we do not attempt to judge the truth or falsity of a claim based on whether it is subjective. Instead, we aim to make a more granular distinction of claims and design more appropriate prompts for the LLMs for each type of claim to generate initial viewpoints. These initial viewpoints are then used as the basis for subsequent debate to derive a final conclusion.

Q3:About "conforms to common knowledge".
The term "terrible" in Figure 1 is indeed part of a supporting comment, but its connection to "common knowledge" is not direct in a logical sense; rather, it is indirectly conveyed through emotional expression. The role of such emotional comments lies in the emotional resonance and its indirect link to common knowledge: comments like "terrible" reflect the widespread societal emotional response to events such as child infections or deaths, aligning with the common psychological reactions people have to similar public health tragedies. Therefore, although it does not provide new factual evidence, it indirectly echoes the common knowledge expressed in the statement "Breaking: A child under the age of 18 has died of coronavirus in Los Angeles, public health officials announce, in a rare and tragic case," through emotional resonance.

Q4:About the comments in determining the truthfulness of a claim.
GPT-3.5 contains factual information about COVID-19, but in Figure 3, the different comments do influence the experimental results. Therefore, the assistance of comments is crucial in determining the veracity of the statement.

Q5:About our model.
We are not simply applying multi-agent debate technology to rumor detection; instead, we have designed a complex strategy that includes Stance Separation, Initial Opinion Generation, and Multi-Agent Debate. This approach involved extensive experimentation before arriving at the current model.

Comments Suggestions And Typos:
The notation $t_i$ is used in Section 4.5 Early Detection, where, by setting different checkpoints, models are assessed using the post count up to each detection point. We used $t_i$ to rank the comments. Thank you for your valuable suggestion; we will provide further clarification on this. Regarding line 399, the references are for datasets.





review3:

Dear Reviewer 4TTR, we sincerely appreciate your invaluable and constructive comments. We respond to your concerns one by one.

Q1: About the definition of Rumour Detection task.

We are very fortunate that you took the time to carefully read our paper and pay attention to the details. The definition of the rumor detection task is presented in Section 3.1 "Problem Formulation" (lines 221-231).

Q2: About the dataset selection.

There are many datasets for rumor detection during breaking events like COVID-19. The Twitter-COVID19 and Weibo-COVID19 datasets are two commonly used datasets in the field of breaking event social media rumor detection. We have mentioned this in Section 4 "Experiment" (lines 398-402) of the paper.

Q3: The paper uses LLMs, the training data of which includes the period of COVID-19.

Thank you very much for raising this valuable concern. As you mentioned, the LLM used in our study includes data from the COVID-19 period. However, our primary focus is on how the method we propose improves performance based on the LLM. This very aspect validates the value of our approach.

Q4:Regarding the examples and error analysis in the experiment.

Your suggestion is reasonable, as it clearly demonstrates how the model understands semantics and generates answers. In the forthcoming public version, we will organize this and include it in the appendix.

Q5: The paper's related work section is missing a lot of existing relevant literature.

Thank you for your valuable suggestion. We will include references to the relevant literature you mentioned：

Karadzhov, G., Vlachos, A., & Stafford, T. (2024). The effect of diversity on group decision-making. arXiv preprint arXiv:2402.01427.

Karadzhov, G., Stafford, T., & Vlachos, A. (2022). What makes you change your mind? An empirical investigation in online group decision-making conversations. arXiv preprint arXiv:2207.12035.

Schlichtkrull, M., Guo, Z., & Vlachos, A. (2024). Averitec: A dataset for real-world claim verification with evidence from the web. Advances in Neural Information Processing Systems, 36.

Dougrez-Lewis, J., Kochkina, E., Liakata, M., & He, Y. (2024, May). Knowledge Graphs for Real-World Rumour Verification. In Proceedings of the 2024 Joint International Conference on Computational Linguistics, Language Resources and Evaluation (LREC-COLING 2024) (pp. 9843-9853).

Kochkina, E., Hossain, T., Logan IV, R. L., Arana-Catania, M., Procter, R., Zubiaga, A., ... & Liakata, M. (2023). Evaluating the generalisability of neural rumour verification models. Information Processing & Management, 60(1), 103116.

Hossain, T., Iv, R. L. L., Ugarte, A., Matsubara, Y., Young, S., & Singh, S. (2020, December). COVIDLies: Detecting COVID-19 misinformation on social media. In Proceedings of the 1st Workshop on NLP for COVID-19 (Part 2) at EMNLP 2020.

Strong, M., Aly, R., & Vlachos, A. (2024). Zero-Shot Fact Verification via Natural Logic and Large Language Models. arXiv preprint arXiv:2410.03341.


